LiRank: Industrial Large Scale Ranking Models at LinkedIn

We present LiRank, a large-scale ranking framework at LinkedIn that brings to production state-of-the-art modeling architectures and optimization methods. We unveil several modeling improvements, including Residual DCN, which adds attention and residual connections to the famous DCNv2 architecture. We share insights into combining and tuning SOTA architectures to create a unified model, including Dense Gating, Transformers and Residual DCN. We also propose novel techniques for calibration and describe how we productionalized deep learning based explore/exploit methods. To enable effective, production-grade serving of large ranking models, we detail how to train and compress models using quantization and vocabulary compression. We provide details about the deployment setup for large-scale use cases of Feed ranking, Jobs Recommendations, and Ads click-through rate (CTR) prediction. We summarize our learnings from various A/B tests by elucidating the most effective technical approaches. These ideas have contributed to relative metrics improvements across the board at LinkedIn: +0.5% member sessions in the Feed, +1.76% qualified job applications for Jobs search and recommendations, and +4.3% for Ads CTR. We hope this work can provide practical insights and solutions for practitioners interested in leveraging large-scale deep ranking systems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix


==> acknowledgements.tex <==
The authors would like to thank Ying Xuan, Zhifei Song, Samaneh Moghaddam, Jerry Shen, Arjun Kulothungun, Praneeth Boda and others who collaborated with us.

==> engagement.tex <==
Since we define system quality by user interaction metrics such as click rate and good click rate (see \S\,\ref{sec:Overview:Metrics}), we want to use historical interaction rates as features to our ranking model. We compute two classes of features for each media document: (1) actual engagement features and (2) predicted engagement features.

Actual engagement features are ratios of historical engagement rates of media: click rate, like rate, save rate, impression rate. In order to reduce noise, we compute these metrics every day averaged over the previous 7 days. Impression rate is defined as the number of times a media was in the application viewport normalized by a constant. Like rate is defined as the number of times a media was liked divided by the impression rate. Save rate and click rate are defined similarly. 

One issue with engagement features is that they can be unreliable for fresh media (i.e.\ cold start problem). To mitigate this problem, we calculate \textit{predicted engagement features}: predicted click rate, predicted like rate, predicted save rate, and predicted impression rate. To calculate predicted engagement we prepared a large pool of seed media (${\sim}100\textrm{M}$) which has been engaged during the week. We used a different pool of seed media for photos and videos because we expect different user engagement behavior for them.
For each seed media in the pool we compute its embedding and engagement features as defined above. When the new target media is deployed we extract its embedding and apply a weighted {\itshape k-nearest neighbors} search to find top-{\itshape K} similar seed media, and then take a weighted average of seed media engagement counters to calculate predicted engagement counter. Weights can be defined as the similarity between the target and seed media embedding. 
We used actual engagement features in the wide \& deep neural network model (defined in \S\,\ref{sec:second_stage_ranking}) and observed a {\bfseries 1.1\%} improvement in good click rate (Table~\ref{tab:metric_gains}) and an additional {\bfseries 0.7\%} improvement in good click rate when using both actual engagement and predicted engagement features.

==> tuning_model_convergence.tex <==
\subsection{Optimization for model convergence}\label{sec:Overview:tuning_model}

Deep neural networks are non-convex in nature and model generalization varies across training runs and hyperparameter settings. We focused on leveraging various optimization algorithms with the dual goals of (a) improved generalization and (b) faster training with large batch sizes in mind. 

Since modern neural networks consist of many parameters and are trained on massive datasets, use of large batches can significantly accelerate the training process. Unfortunately, empirical evidence suggests that large-batch training converges to \textbf{sharper} minima, often correlated with poorer performance on test data (drop in generalization performance)~\cite{keskar2016large}. Sharpness can be defined in several ways; a popular approach is to study the eigenvalues of the Hessian of the loss function. Several empirical studies explore the importance of hyperparameters in large batch training \cite{Goyal2017, shallue2018measuring, hoffer2017train} but a solution that works across domains and tasks remains elusive.

For RecSys, faster training can lead to models that adapt well to varying training data distribution. Such quick adaptation can positively impact business metrics in applications such as newsfeed and ads recommendations \cite{ramanath2021lambda}. However, careful optimization routines must be adopted in large-batch training, as na\"ive training can adversely affect generalization performance.

\textbf{Large-batch training for CV and NLP} Initial inroads into improving the generalization performance of large-batch training were made in the domain of computer vision. Learning rate scheduling plays an important role in scaling effectively to large batch sizes and recently many heuristics like linear or square root scaling of learning rate \cite{krizhevsky2014one, you2019LEGW} and gradual warm up of learning rate \cite{you2019large, Goyal2017} have been used to close the generalization gap at large batch sizes for computer vision models. Using gradual learning rate warmup, authors of \cite{Goyal2017} scale the batch size of an image classification model to $\approx$8k on the ImageNet dataset \cite{deng2009imagenet, krizhevsky2012imagenet}. More recently, new optimizers have been devised to leverage functionality like adaptive per-layer scaling to scale batch sizes to even larger values \cite{you2017large, you2019large, yamazaki2019yet} for computer vision models. 


\textbf{Large-batch training for RecSys} While most of the recent developments for large-batch training have happened for CV and NLP-related DNNs, deep RecSys models have received little consideration towards effective large-batch training. Compared to CV/NLP, RecSys dataset labels are noisier and the models are often under-parameterized. Therefore, many RecSys DNNs need tailored optimization setups. For instance, AdaGrad \cite{duchi2011adaptive} is particularly successful for RecSys DNN training using datasets with sparse categorical features \cite{yao2021adahessian, naumov2019deep}. Modern RecSys DNNs typically contain embeddings in conjunction with a single or dual-tower network \cite{guo2017deepfm, wang2017deep, wang2021dcn, he2017neural}
 and can contain a very large number of parameters. 

\textbf{Gradient clipping and learning rate warm up} Both learning rate warm up and gradient clipping are effective techniques for stabilizing deep model training. Learning rate warm up has recently been used to stabilize training of small-batch Adam \cite{kingma2014adam} for NLP models \cite{liu2019variance}, as well as reducing the generalization gap for large-batch training \cite{you2019LEGW, you2017large, you2019large}. Gradient clipping \cite{pascanu2013difficulty} has been used to stabilize training with SGD \cite{zhang2019gradient} and adaptive optimizers \cite{brown2020language, chen2021vision}. Recent evidence has emerged for how learning rate warm up and gradient clipping help avoid regions of high curvature during early stages of optimization and guide the solution towards flatter regions \cite{gilmer2021loss} (flatter regions are correlated with better generalization performance \cite{keskar2016large}).

\textbf{Our Learnings} Our experimentation revealed that different models require varying optimization setups. While Adam worked well for most setups, we had to leverage AdaGrad for models where the number of sparse features was high. This had a large impact on model performance. At the same time, we made extensive use of learning rate warm up and gradient clipping to improve model generalization at large batch sizes. Specifically, we always warm up the learning rate for large batch training and clip the global gradient to have unit norm for all experiments. For warm up, we use a simple rule of thumb of doubling the fraction of steps used to increase the learning rate to a peak whenever the batch size is doubled, capping the increase to 60\% of total training steps. This allowed us to significantly improve generalization performance across all settings as well as close the generalizaiton gap at large batch sizes.
